An analysis of the graph processing landscape

The value of graph-based big data can be unlocked by exploring the topology and metrics of the networks they represent, and the computational approaches to this exploration take on many forms. The use-case of performing global computations over a graph, it is first ingested into a graph processing system from one of many digital representations. Extracting information from graphs involves processing all their elements globally, and can be done with single-machine systems (with varying approaches to hardware usage), distributed systems (either homogeneous or heterogeneous groups of machines) and systems dedicated to high-performance computing (HPC). We provide an overview of different aspects of the graph processing landscape and describe classes of systems based on a set of dimensions we detail. The dimensions we detail encompass paradigms to express graph processing, different types of systems to use, coordination and communication models in distributed graph processing, partitioning techniques and different definitions related to the potential for a graph to be updated. This survey is aimed at both the experienced software engineer or researcher as well as the newcomer looking for an understanding of the landscape of solutions (and their limitations) for graph processing.

==> definitions.tex <==
%%%%%%%%%%
%%%%%%%%%% PUBLICATION NAMES
%%%%%%%%%%
\newcommand{\veilgraph}{{\scshape VeilGraph}\xspace}
\newcommand{\gellyscheduling}{{\scshape Gelly-Scheduling}\xspace}


%%%%%%%%%%
%%%%%%%%%% THESIS COMMANDS
%%%%%%%%%%
\newcommand\footurl[6]{%
  \footnote{{\texttt{#1} #2. Access date: #3 #4 '#5. \url{#6}}}%
}

%%%%%%%%%%
%%%%%%%%%% FONTS
%%%%%%%%%%
\RequirePackage{fix-cm}

\DeclareFontFamily{U}{rsfs}{\skewchar\font127 }
\DeclareFontShape{U}{rsfs}{m}{n}{%
   <-6> rsfs5
   <6-8> rsfs7
   <8-> rsfs10
}{}


%%%%%%%%%%
%%%%%%%%%% lstlistings - Cypher query language aesthetics
%%%%%%%%%%

\definecolor{keyword}{HTML}{2771a3}
\definecolor{pattern}{HTML}{b53c2f}
\definecolor{string}{HTML}{be681c}
\definecolor{relation}{HTML}{7e4894}
\definecolor{variable}{HTML}{107762}
\definecolor{comment}{HTML}{8d9094}


\lstdefinestyle{CypherStyle}{
	numbers=none,
	stepnumber=1,
	numbersep=5pt,
	basicstyle=\small\ttfamily,
	keywordstyle=\color{keyword}\bfseries\ttfamily,
	commentstyle=\color{comment}\ttfamily,
	stringstyle=\color{string}\ttfamily,
	identifierstyle=,
	showstringspaces=false,
	aboveskip=3pt,
	belowskip=3pt,
	columns=flexible,
	keepspaces=true,
	breaklines=true,	
	captionpos=b,
	tabsize=2,
	frame=none,
}

\lstdefinelanguage{cypher}
{
	morekeywords={
		MATCH, OPTIONAL, WHERE, NOT, AND, OR, XOR, RETURN, DISTINCT, ORDER, BY, ASC, ASCENDING, DESC, DESCENDING, UNWIND, AS, UNION, WITH, ALL, CREATE, DELETE, DETACH, REMOVE, SET, MERGE, SET, SKIP, LIMIT, IN, CASE, WHEN, THEN, ELSE, END,
		INDEX, DROP, UNIQUE, CONSTRAINT, EXPLAIN, PROFILE, START,
	}
}


\newcommand{\mycdots}{\cdot\!\cdot\!\cdot}
\lstset{language=cypher,
	literate=*
	{...}{$\mycdots$}{1}
	{theta}{$\theta$}{1}
}

%%%%%%%%%%
%%%%%%%%%% lstlistings - Java language aesthetics
%%%%%%%%%%

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

%\lstdefinestyle{JavaStyle}{
%  aboveskip=3mm,
%  belowskip=3mm,
%  showstringspaces=false,
%  columns=flexible,
%  keywords=[2]{String,ExecutionEnvironment,Graph,NullValue,Long,PageRank,DataSet,Result},
%  basicstyle={\small\ttfamily},
%  numbers=none,
%  numberstyle=\tiny\color{gray},
%  keywordstyle=\color{blue},
%  keywordstyle=[2]\color{mauve},
%  commentstyle=\color{dkgreen},
%  stringstyle=\color{mauve},
%  breaklines=true,
%  breakatwhitespace=true,
%  tabsize=3,
%  upquote=true,
%  literate={``}{\textquotedblleft}1,
%  deletestring=[b]",
%    ,
%}

\lstset{frame=tb,
  language=Java,
  aboveskip=3mm,
  belowskip=3mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\small\ttfamily},
  numbers=none,
  numberstyle=\tiny\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3
}


%%%%%%%%%%
%%%%%%%%%% TikZ shapes and colors
%%%%%%%%%%

\def\notcheckmark{
\begin{tikzpicture}
\draw[scale=0.4, fill=black](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;
\draw[line width=1pt] (.15, .30) -- (.4, .1);
\end{tikzpicture}
}

\def\checkmark{
\begin{tikzpicture}
\draw[scale=0.4, fill=black](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;
\end{tikzpicture}
}

\def\crossmark{
\begin{tikzpicture}
\draw[scale=0.4, fill=black, line width=1.0pt](0,.65) -- (.5,0)  -- cycle;
\draw[scale=0.4, fill=black, line width=1.0pt](0,0) -- (.5,.65)  -- cycle;
\end{tikzpicture}
}


\DeclareRobustCommand{\bluecirclemarker}{\raisebox{0.5pt}{\tikz{\node[draw,scale=0.4,circle,fill=black!20!blue](){};}}}
\DeclareRobustCommand{\triangledownmarker}{\raisebox{0pt}{\tikz{\node[draw,scale=0.3,regular polygon, regular polygon sides=3,fill=black!45!green,rotate=180](){};}}}
\DeclareRobustCommand{\triangleupmarker}{\raisebox{0.5pt}{\tikz{\node[draw,scale=0.3,regular polygon, regular polygon sides=3,fill=black!10!red,rotate=0](){};}}}
\DeclareRobustCommand{\squaremarker}{\raisebox{0.5pt}{\tikz{\node[draw,scale=0.4,regular polygon, regular polygon sides=4,fill=none](){};}}}
\DeclareRobustCommand{\diamondmarker}{\raisebox{0pt}{\tikz{\node[draw,scale=0.4,diamond,fill=black!10!gray](){};}}}
\DeclareRobustCommand{\blackcirclemarker}{\raisebox{0.6pt}{\tikz{\node[draw,scale=0.4,circle,fill=black!100!](){};}}}

%%%%%%%%%%
%%%%%%%%%% Misc. commands.
%%%%%%%%%%

% Key-value store structures in LaTeX:
% https://tex.stackexchange.com/questions/48907/global-key-value-dictionary
% Key-values with \usepackage{pgfkeys}:
% ftp://ftp.di.uminho.pt/pub/ctan/graphics/pgf/base/doc/pgfmanual.pdf

% How to inserting parts of a reference (year, author name, etc.) in text using biblatex and without natbib:
% https://tex.stackexchange.com/questions/109940/citing-author-or-year-only-without-natbib
%\newcommand{\system}[4]{\textbf{\texttt{#1}} -- \textit{#2 #3}~\cite{#4}}
\newcommand{\system}[4]{\textbf{\texttt{#1}}, \textit{#2}~\cite{#4}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LaTeX Overlay Generator - Annotated Figures v0.0.1
% Created with http://ff.cx/latex-overlay-generator/
% If this generator saves you time, consider donating 5,- EUR! :-)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand*\annotatedFigureBoxCustom[8]{\draw[#5,thick,rounded corners] (#1) rectangle (#2);\node at (#4) [fill=#6,thick,shape=rectangle,draw=#7,inner sep=2pt,font=\sffamily,text=#8] {\textbf{#3}};}
\newcommand*\annotatedFigureBox[4]{\annotatedFigureBoxCustom{#1}{#2}{#3}{#4}{white}{white}{black}{black}}
\newcommand*\annotatedFigureText[4]{\node[draw=none, anchor=south west, text=#2, inner sep=0, text width=#3\linewidth,font=\sffamily] at (#1){#4};}
\newenvironment {annotatedFigure}[1]{\centering\begin{tikzpicture}
\node[anchor=south west,inner sep=0] (image) at (0,0) { #1};\begin{scope}[x={(image.south east)},y={(image.north west)}]}{\end{scope}\end{tikzpicture}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





